Sada-ASR: A Production Multidialectal Arabic Speech Recognition System

Callers to Arabic customer-service lines speak their own dialect, while speech recognizers are built and evaluated mainly on Modern Standard Arabic (MSA). A recognizer that mishears the dialect breaks the call before anything else can help. We present Sada-ASR, the speech recognizer of EchoNova's production Arabic voice agent. On a 120-hour test set of MSA and eight dialects, it has the lowest word and character error rates of twelve systems, against eleven from Microsoft, ElevenLabs, Google, OpenAI, Speechmatics, IFM, Cohere, NVIDIA and Audar: 11.69% word error rate against 13.51% for the strongest, Microsoft's MAI-Transcribe-2 (a lead of 0.74 points on clips unaffected by that system's fixed number and script conventions), and 15.52% against 16.96% averaged over varieties. Its largest margins are on Omani (4.30 points), Egyptian (3.78) and Saudi (2.19) speech; it is level on Syrian and loses on Lebanese (24.96% against 23.05%), mostly because it writes Lebanese words in MSA forms and is less verbatim. On six public test sets its average word error rate under the leaderboard's current scoring is 17.17%, below every published figure we found, among them Falcon-ASR (20.92%), Jais-ASR (22.85%) and Audar-ASR-V1-Turbo (23.17%), though none of these states that it used that scoring, so the comparison is indicative. We describe the data pipeline and methodology behind Sada-ASR and release a 20-hour subset of the test set with our scoring code.

==> macros.tex <==
\newif\ifdraft
\draftfalse

\definecolor{fillred}{RGB}{190,20,30}
\definecolor{verifyamber}{RGB}{190,105,0}
\definecolor{noteblue}{RGB}{20,80,170}

\ifdraft
  \newcommand{\fillin}[2]{\textcolor{fillred}{\textbf{[#1:}~#2\textbf{]}}}
  \newcommand{\verify}[1]{\textcolor{verifyamber}{#1\textsuperscript{\,?}}}
  \newcommand{\note}[1]{\textcolor{noteblue}{\textit{[#1]}}}
\else
  \newcommand{\fillin}[2]{\PackageError{draft}{Unfilled placeholder (#1): #2}{}}
  \newcommand{\verify}[1]{\PackageError{draft}{Unverified text: #1}{}}
  \newcommand{\note}[1]{\PackageError{draft}{Authoring note left in: #1}{}}
\fi

\newcommand{\sys}{EchoNova Sada}
\newcommand{\asr}{Sada-ASR}
\newcommand{\sadacorpus}{the SADA corpus}

\makeatletter
\@ifpackageloaded{babel}{%
  \RequirePackage{accsupp}%
  \DeclareRobustCommand{\ar}[1]{\BeginAccSupp{method=pdfstringdef,unicode,ActualText={#1}}%
    \foreignlanguage{arabic}{\textRL{#1}}\EndAccSupp{}}%
}{%
  \newcommand{\ar}[1]{\textcolor{fillred}{[AR]}}%
}
\makeatother

\newcommand{\best}[1]{\textbf{#1}}
\newcommand{\ours}{\rowcolor{black!6}}

\urlstyle{same}
\makeatletter
\g@addto@macro{\UrlBreaks}{\do\-}
\makeatother

\newcommand{\linkicon}[1]{\raisebox{-0.18em}{\includegraphics[height=1.05em]{figures/icons/#1.pdf}}\,}

\definecolor{seriesblue}{HTML}{2A78D6}
\definecolor{inksecondary}{HTML}{52514E}

